Workflow Provenance in the Lifecycle of Scientific Machine Learning

Machine Learning (ML) has already fundamentally changed several businesses. More recently, it has also been profoundly impacting the computational science and engineering domains, like geoscience, climate science, and health science. In these domains, users need to perform comprehensive data analyses combining scientific data and ML models to provide for critical requirements, such as reproducibility, model explainability, and experiment data understanding. However, scientific ML is multidisciplinary, heterogeneous, and affected by the physical constraints of the domain, making such analyses even more challenging. In this work, we leverage workflow provenance techniques to build a holistic view to support the lifecycle of scientific ML. We contribute with (i) characterization of the lifecycle and taxonomy for data analyses; (ii) design principles to build this view, with a W3C PROV compliant data representation and a reference system architecture; and (iii) lessons learned after an evaluation in an Oil & Gas case using an HPC cluster with 393 nodes and 946 GPUs. The experiments show that the principles enable queries that integrate domain semantics with ML models while keeping low overhead (<1%), high scalability, and an order of magnitude of query acceleration under certain workloads against without our representation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> our-contents/algorithms/instrumented_code.tex <==

\begin{center}
\begin{minipage}[t]{0.7\textwidth}
\begin{lstlisting}[
    language=python,
    caption={Excerpt of provenance capture in an exemplary ML training script.},
    label={listing:trainingscript}
]
from provenance_lib import learning
prov.init('learning_workflow')
...
prov.capture_in('training', training_settings, input_data_references)
for e in range(1, max_epochs):
  prov.capture_in('epoch', e)
  ...
  for batch_id in data_batches:
      prov.capture_in('batch', batch_id)
      ...
      prov.capture_out('batch', loss_value;
  prov.capture_out('epoch', confusion_matrix, model_hyperprms, model_perf, model_ref)
prov.capture_out('training');
prov.close();

\end{lstlisting}
\end{minipage}
\end{center}




==> our-contents/algorithms/query.tex <==

\begin{algorithm}
  \DontPrintSemicolon
  
  \KwIn{
  
  \begin{enumerate}[label=\textbullet,wide,labelindent=0mm] 
  
    \item $Project$: Set of attributes to project, \textit{s.t.} $P = \{(R,a) | R \in D \text{ and } a \in \mathscr{S}(R)$, where:
        
        \begin{enumerate}[label=-,wide,labelindent=3mm]
            \item $D = \{Domain\_Data, Data\_Preparation, Learning\_Data, Learning, Model \}$ and 
            
            \item $\mathscr{S}(R) \text{ is the schema of } R$.
        \end{enumerate}
        
    \item $Filter$: Set of minterm predicates to filter results, \textit{s.t.} $M = \{ (a, \theta, v)\}$,     where:
    
        \begin{enumerate}[label=-,wide,labelindent=3mm]
         \item $a \in \mathscr{S}(R) \text{ and } R \in D$,
         \item $\theta \in \{=,<,\neq,\leq,>,\geq  \} \text{ and, }$
         \item $v$ is either a value from the domain of $a$ or it the result of another \codefont{PROV-ML Query} (\ie{} a subquery), whose result set has the domain of $a$.
        \end{enumerate}


    \item $(S,R)$: $S \in D$ and $R \in D$ are the source and destination relations, respectively, in \codefont{PROV-ML Queries}.

    \item $Aggregate$: Optional argument to specify a set of aggregate functions, \textit{s.t.}
        $F = \{f(a) |$ 
                $f \in \{$\codefont{avg}$,$ \codefont{max} $, ...\}$ and
            $a \in \mathscr{S}(R), R \in D\}$
   
  \end{enumerate}
  
  }
  
  \KwOut{Result Set}
  
  \algrule
  
  \codefont{prov.query(}
        
        \qquad \codefont{filter=}$M$,   
        
        \qquad \codefont{project=}$P$,  
        
        \qquad \codefont{aggregate=}$F$,
        
        \qquad \codefont{source=}$S$,
        
        \qquad \codefont{dest=}$R$
   
  
\codefont{)}
  
  
  

 \caption{\codefont{PROV-ML Query} Definition}
 \label{alg:alg_tune_operator}

\end{algorithm}



==> our-contents/algorithms/query_building_defs.tex <==

\noindent
\createDDP{dp:provenance-query}{Easing Provenance Query Specification and Query Building with  Relational Algebra and Graphs}
As characterized in Section \ref{sec:ml_lifecycle}, the provenance analyses are traversal queries on a provenance graph and with analytical features (\eg{} aggregations). 
However, since the \MLView{} has detailed information on several computational processes and data, querying it may not be trivial, and thus with this design principle, we provide a standardized, generic way to declaratively express provenance queries over the \MLView{} based on its conceptual data schema, to facilitate both query specification and query building.
To enable query specification to the \MLView{}, let us first represent its conceptual data schema using relational algebra and a directed graph.
Using relational algebra, the seven key concepts in the conceptual data schema becomes relations and the \textit{n:m} relationship named \codefont{UsedDomainData} becomes an extra relation.
Using a directed graph, let $G = (V,E)$ be the directed graph with the relational representation of the
\MLView{}'s conceptual data schema, 
where the vertices $V = \{R_1, ..., R_8\}$ are the relations and the edges $E$ are the relationships. The direction of an edge $(R_i, R_j) \in E$ means that $R_j$ has an attribute that references an attribute of $R_i$. Figure \ref{fig:simplemodel}(B) illustrates this graph representation showing how it matches the conceptual data schema in Figure \ref{fig:simplemodel}(A). Then, we can define the specification of a provenance query for the lifecycle as follows.


% \begin{mydef}{def:relationalgraph}{Relational Graph}
% A \textit{Relational Graph} $G$ is a directed graph to constitute the provenance data in the \MLCycle{}, with its main concepts (represented as \textit{relations} from the relational algebra) and their relationships. 
% It is represented as $G = (V,E)$, such that
% $V = \{DomainData, UsedDomainData, DataPreparation, LearningData, Learning, Model \}$ and
% $E = \{(R_i,R_j) | (R_i,R_j) \in V^2 \text{, } R_i \neq R_j \text{, and } R_j \text{ \textit{references} } R_i\}$.
% \end{mydef}


\input{our-contents/algorithms/query_definition.tex}

Given the query specification, a provenance system needs to build the query that will be ultimately executed by the underlying DBMS that physically stores the \MLView{}.
Concrete examples of some of the queries \queries{} are in the Table \ref{tab:provmlqueries}.
The most complex part of building a $ProvMLQuery$ is to determine the path through which the query will traverse.
Based on the inputs of the $ProvMLQuery$ specification, 
the query path will be the longest path possible among all relations in $Project$ and $Filter$.
It is well-known that finding the longest path in a generic graph is hard, but it is trivial in a directed acyclic graph (DAG).
Thus, we first define a DAG, named \textit{path graph}, with all possible paths (\ie{} a complete directed graph but with edges going in only one direction) between the relations in the relational representation graph $G$ of the \MLView{}'s conceptual data schema as follows. Fig.~\ref{fig:simplemodel}(C) illustrates the path graph.

\begin{mydef}{def:pathgraph}{Path Graph}
Let $\Gamma' = (V, \mathscr{E}')$ be the complete directed graph formed by the vertices $V$ of $G$.
The \textit{Path Graph} $\Gamma$ is the subgraph 
of $\Gamma'$ but only with the edges going in the forward direction, given the topological order, thus forming a DAG.
That is, 
$\Gamma = (V, \mathscr{E})$, such that
$\mathscr{E} = \{(R_i, R_j) | (R_i, R_j) \in \mathscr{E}' \text{ and } j > i\}$. 

\end{mydef}

Finally, we can define the provenance query path as the natural join of all relations in $Project$ and $Filter$, joining in the longest path, as follows:

\begin{mydef}{def:naturalpath}{Provenance Query Path}
The \textit{Provenance Query Path} $\mathscr{P}$ for a given $ProvMLQuery(Project,Filter)$ is the natural joins of the relations in the longest path found in the subgraph $S$ of the  Path Graph $\Gamma$, where the set of vertices of $S$  is formed by all relations in $Project$ and $Filter$.
That is, $\mathscr{P}(Project,Filter) = (R_i \bowtie R_{i+1} \bowtie ... \bowtie R_k)$, such that $\{R_i, R_{i+1}, ..., R_k\}$ is the longest path of $S$.
\end{mydef}

\noindent The join clauses in $\mathscr{P}$ are omitted for the sake of simplicity, but they are obtained using the attributes represented by the reference edges in 
the relational representation graph $G$ of the \MLView{}'s conceptual data schema.




==> our-contents/algorithms/query_definition.tex <==


\begin{mydef}{def:provquery}{Provenance Query Specification for the \MLCycleCammel{}}
The specification of a provenance query over the \MLCycle{} ($ProvMLQuery$) provides the structure for the minimum input required to build the provenance query that will be executed over the \MLView{}. A $ProvMLQuery$ is specified as:
$$ResultSet \leftarrow ProvMLQuery(Project,Filter) \text{, where:}$$

\begin{enumerate}[label=\textbullet,wide,labelindent=0mm,nolistsep]

\item $Project$: Set of attributes to project, defined as $Project = \{(f,R.a)\}$, such that:
    \begin{enumerate}[label=-,wide,labelindent=3mm,nolistsep]
        \item $f \in \{$  \codefont{avg}, \codefont{max}, \codefont{count}, ...$\}$ is an optional argument used when the query needs an aggregate function,
        
        \item $R$ is a relation that maps to one of the key concepts in the \MLView{}'s conceptual data model,
        
        \item $a \in \mathscr{S}(R)$ is an attribute of $R$ and $\mathscr{S}(R)$ is the schema of $R$.
        %Nao precisa da tabela que resolve o n:m aqui porque nunca a expomos pro usuario consultar. Ela so serve pro resolvedor da consulta
        
    \end{enumerate}

\item $Filter$: Set of minterm predicates to filter results, defined as  $Filter = \{ (R.a \ \theta \ v)\}$, such that:

    \begin{enumerate}[label=-,wide,labelindent=3mm,nolistsep]
     \item $a \in \mathscr{S}(R)$ and $R$ is a relation that maps to a concept in \MLView{}'s conceptual data model,
     \item $\theta \in \{=,<,\neq,\leq,>,\geq \} \text{, and }$
     \item $v$ is either a value from the domain of $R.a$ or it the result of another $ProvMLQuery$ (\ie{} a subquery), whose result set has the domain of $R.a$.
    \end{enumerate}

% Source e Destination sao opcionais. Por ex, 'select min(loss) where model.learning_data = 2' nao exige source e destination. 
% \item $Source \in DB$ and $Destination \in DB$ are optional arguments, used to specify the source and destination relations, respectively, when the query does a graph traversal over the relations in $DB$.

% \item $Aggregate$: Optional argument to specify a set of aggregate functions, \textit{s.t.}
%     $F = \{f(R.a) |$ 
%             $f \in \{$\codefont{avg}$,$ \codefont{max} $, ...\}$ and
%         $a \in \mathscr{S}(R), R \in DB\}$.

\end{enumerate}

\end{mydef}

==> our-contents/tables/pqml_queries.tex <==

\begin{table}[ht]
\footnotesize
\caption{Examples of $PorvMLQueries$.}
\label{tab:provmlqueries}
\topsepremove
\begin{tabular}
{
m{.05\textwidth}|
m{.6\textwidth}|
m{.25\textwidth}
}
\rowcolor{table_header}
\textbf{$PQML_i$} &
\textbf{$PQML$ Arguments} &
\textbf{SQL-like Illustration}
\\
\toprule
\rowcolor{table_row_even}
{$PQML_1$} &
$Project = \{$
    $\begin{aligned}[t]
    &DomainData.geographicCoordinates, DomainData.oilBasin, \\
    &DomainData.oilField, \\ 
    &DomainData.numberSeismicSlices \ \}
    \end{aligned}$

$
Filter = (
     Model.id = \text{`given model id'} 
    )
$
&
\codefont{SELECT} 

\hskip 1em $DomainData.geographicCoordinates,$

\hskip 1em $DomainData.oilBasin,$

\hskip 1em $DomainData.oilField,$

\hskip 1em $DomainData.numberSeismicSlices$

\codefont{FROM} $DB$

\codefont{WHERE} $Model.id = \text{`given model id'}$ 
\\ 
\rowcolor{table_row_odd}
{$PQML_2$}
&
$Project = \{$
    $\begin{aligned}[t]
    &DataPreparation.tileSize, DataPreparation.noiseFilterThreshold, \\
    &LearningData.seismicRanges \ \}
    \end{aligned}$

$
Filter = (
     Model.id = \text{`given model id'} 
    )
$
&
\codefont{SELECT} 

\hskip 1em $DataPreparation.tileSize,$

\hskip 1em $DataPreparation.noiseFilterThreshold,$

\hskip 1em $LearningData.seismicRanges$

\codefont{FROM} $DB$

\codefont{WHERE} $Model.id = \text{`given model id'}$ 
\\ 
\rowcolor{table_row_even}
{$PQML_3$} & 
$
Project = \{
    Model.evaluation,
    Learning.hyperparameters
    \} 
$

$Filter = \{$
    $\begin{aligned}[t]
    &(LearningData.id = \text{`given learning data id'}), \\
    &(Model.loss = PQML_{31}(Project=(min,Model.loss),\\
            & \hskip 11.0em Filter=(Model.learningDataId = \text{`given learning data id'}))\\
            & )
    &\\
    \end{aligned}$
&
\codefont{SELECT} 

\hskip 1em $Model.evaluation,$

\hskip 1em $Learning.hyperparameters$

\codefont{FROM} $DB$

\codefont{WHERE} $Model.learningDataId = \text{`id'}$ 

\codefont{AND} $Model.loss = ($

\hskip 1em \codefont{SELECT min($Model.loss$)}

\hskip 1em \codefont{FROM DB}

\hskip 1em \codefont{WHERE} $Model.learningDataId = \text{`id'}$)
\\ 
\rowcolor{table_row_odd}
$PQML_4$ &
$Project = \{$
    $\begin{aligned}[t]
    &\hskip -0.1em Learning.epoch, (avg, Learning.epoch.batch.elapsedTime),\\
    &\hskip -0.5em (min, Learning.epoch.batch.elapsedTime),(max, Learning.epoch.batch.elapsedTime) \ \}
    \end{aligned}$

$
Filter = (
     LearningData.id = \text{`given model id'} 
    )
$
&
\codefont{SELECT} 

\hskip 1em $Learning.epoch,$

\hskip 1em $avg(Learning.epoch.batch.elapsedTime),$

\hskip 1em $max(Learning.epoch.batch.elapsedTime),$

\hskip 1em $min(Learning.epoch.batch.elapsedTime)$

\codefont{FROM} $DB$

\codefont{WHERE} $LearningData.id = \text{`id'}$ 

\codefont{GROUP BY} $Learning.epoch$
\\ 
\rowcolor{table_row_even}
$PQML_5$ &
$Project = \{$
    $\begin{aligned}[t]
    &Learning.epoch,\\
    &(avg, Learning.epoch.batch.elapsedTime),\\
    &Model.evaluation \ \}
    \end{aligned}$

$
Filter = (
     DataPreparation.seismicRanges = \text{`given ranges'} 
    )
$
&
\codefont{SELECT} 

\hskip 1em $Learning.epoch,$

\hskip 1em $Learning.learningDataId,$

\hskip 1em $Model.evaluation,$

\hskip 1em $avg(Learning.epoch.batch.elapsedTime)$

\codefont{FROM} $DB$

\codefont{WHERE} $DataPreparation.seismicRanges = \text{`given ranges'}$ 

\codefont{GROUP BY}

\hskip 1em $Learning.epoch,Model.evaluation,$ 

\hskip 1em $Learning.learningDataId$
\\ 
\rowcolor{table_row_odd}
$PQML_6$ &
$Project = \{$
    $\begin{aligned}[t]
    &DomainData.filePath,DomainData.numberSeismicSlices,\\
    &DomainData.oilBasin, DomainData.oilField \ \}
    \end{aligned}$

$
Filter = (
     LearningData.id = \text{`given learning data id'}
    )
$
&
\codefont{SELECT} 

\hskip 1em $DomainData.filePath,$

\hskip 1em $DomainData.numberSeismicSlices,$

\hskip 1em $DomainData.oilBasin$

\codefont{FROM} $DB$

\codefont{WHERE} $LearningData.id = \text{`id'}$ 
\\
% \hline
% \hline
\arrayrulecolor{table_row_even}\hline
\end{tabular}
\label{tab:queryexample}
\end{table}



==> our-contents/tables/prov_ml_table_backup.tex <==
% V4
\begin{table}[ht]
\footnotesize
\caption{PROV-ML data representation classes.}
% \begin{tabular}{>{\centering\arraybackslash}m{3.25cm}m{4.5cm}}
\topsepremove
 \begin{tabular}{>{\arraybackslash}m{0.20\textwidth}m{0.80\textwidth}}
% \hline
% \hline
\rowcolor{table_header}
\textbf{Class} & \textbf{Description} \\
\toprule
Study & Investigation (\eg{} research hypothesis) leading ML workflow definitions.
\\ 
\rowcolor{table_row_even}
LearningExperiment & The set of analyses (\eg{} research questions) that drives the ML workflow. 
\\ 
\rowcolor{table_row_odd}
LearningProcessExecution & An ML workflow execution. This is equivalent to \codefont{mls:Run} and was renamed to explicitly preserve the aspects of retrospective provenance, which are not explicitly handled in MLS. 
\\
\rowcolor{table_row_even}
LearningTask and LearningTaskValue & Defines the goal of a learning process, \ie{} the ML task  (\eg{} \codefont{LearningTask}: \textit{Classification}; \codefont{LearningTaskValue}: \textit{Seismic Stratigraphic Classification}). 
\\ 
\rowcolor{table_row_odd}
BaseLearningStage and BaseLearningStageExecution & Abstract classes of \codefont{LearningStage} and \codefont{LearningStageSection}, and their execution counterparts used to conserve them the relationships among other classes while granting them to have special characteristics.
\\
\rowcolor{table_row_even}
LearningStage and LearningStageExecution & Defines a \codefont{Training} or \codefont{Validation} or \codefont{Evaluation}) learning stage and its execution.
\\ 
\rowcolor{table_row_odd}
LearningStageSection \  and \newline 
LearningSectionExecution & Introduces the sectioning semantics, \ie{} capabilities for provenance of subparts of the learning stage and corresponding data.
\\ 
\rowcolor{table_row_even}
LearningDatasetReference and LearningDataset & Defines the dataset to be used by a \codefont{LearningStage} or \codefont{LearningStageSection}. In the last case, it is a section of a \codefont{LearningDatasetReference}. \codefont{LearningDataset} is the dataset used in the execution.
\\ 
\rowcolor{table_row_odd}
DatasetCharacteristic and DatasetCharacteristcValue & Defines metadata about the \codefont{LearningDatasetReference} (\eg{} \#instances),  and \codefont{DatasetCharacteristcValue} relates with a \codefont{LearningDataset} (\eg{} \#instances =8).                      
\\ 
\rowcolor{table_row_even}
FeatureExtraction and FeatureExtractionExecution & Defines the prospective and retrospective feature retrieval process, respectively.  
\\
\rowcolor{table_row_odd}
FeatureSet and FeatureSetData & Defines the features and feature values a \codefont{FeatureExtraction} should generate over  \codefont{LearningDatasetReference}.
\\ 
\rowcolor{table_row_even}
FeatureSetCharacteristic  & Defines the set of metadata that describes the \codefont{FeatureSet} (\eg{} number of features, features' type).                                  
\\ 
\rowcolor{table_row_odd}
Software & Defines a collection of ML techniques' implementations (\eg{} Scikit-Learn).                                                 
\\ 
\rowcolor{table_row_even}
Algorithm & ML technique with no associated technology, software or implementation (\eg{} k-means clustering technique).        
\\ 
\rowcolor{table_row_odd}
Implementation & Defines the retrospective aspect of an \codefont{Algorithm}, \ie{} an ML technique's implementation in a software (\eg{} Scikit-Learn's k-means implementation).                               
\\ 
\rowcolor{table_row_even}
ImplementationCharacteristicValue & Defines the implementation's set of metadata (properties and values),\eg{} version, git hash.    
\\ 
\rowcolor{table_row_odd}
LearningHyperparameter & Defines the prior parameter of an \codefont{Algorithm} used by a \codefont{LearningStage} or \codefont{LearningStageSection}.
\\ 
\rowcolor{table_row_even}
LearningHyperparameterValue & Defines the parameter values of an execution (\eg{} the $k$ value in a k-means clustering technique, range of epochs in a neural network training).                                   
\\ 
\rowcolor{table_row_odd}
ModelSchema & The scope of the resulting model.                                                         
\\ 
\rowcolor{table_row_even}
ModelProspection and Model & The resulting model a \codefont{LearningStage} or a \codefont{LearningStageSection} should generate, and the generated value (\eg{} the trained model after the training stage).                                                                       
\\ 
\rowcolor{table_row_odd}
ModelHyperparameter and ModelHyperparameterValue    &  Hyperparameters a \codefont{LearningStage} or a \codefont{LearningStageSection} generate, and their values corresponding to the resulting model (\eg{} the epoch which the resulting model was generated).               
\\ 
\rowcolor{table_row_even}
DataStoreInstance & Storage of the resulting model.                                    
\\ 
\rowcolor{table_row_odd}
EvaluationMeasure and ModelEvaluation & A measure a \codefont{LearningStage} or a \codefont{LearningStageSection} should evaluate and the generated value (\eg{} the precision of classifier model).                                                                                
\\ 
\rowcolor{table_row_even}
EvaluationSpecification and EvaluationProcedure & Classes directly inherited from MLS, with their semantics preserved. \\
% \hline      
% \hline
\arrayrulecolor{table_row_odd}\hline
\end{tabular}
\label{tab:provlakeml-classes}
\end{table}

